Many-body Approximation for Non-negative Tensors

We present an alternative approach to decompose non-negative tensors, called many-body approximation. Traditional decomposition methods assume low-rankness in the representation, resulting in difficulties in global optimization and target rank selection. We avoid these problems by energy-based modeling of tensors, where a tensor and its mode correspond to a probability distribution and a random variable, respectively. Our model can be globally optimized in terms of the KL divergence minimization by taking the interaction between variables (that is, modes), into account that can be tuned more intuitively than ranks. Furthermore, we visualize interactions between modes as tensor networks and reveal a nontrivial relationship between many-body approximation and low-rank approximation. We demonstrate the effectiveness of our approach in tensor completion and approximation.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> sections/LBTC.tex <==

\begin{wrapfigure}{r}{0.4\textwidth}
\includegraphics[width=0.99\linewidth]{figs/fig_bands.pdf} 
\vspace{-15pt}
\caption{$em$-algorithms.}
\vspace{-25pt}
\label{fig:bands}
\end{wrapfigure}

\section{Application for tensor completion}

Throughout the above discussion, we have proposed interaction as a new measure of tensor to stable decomposition. By replacing the traditional low-rank approximation with many-body approximation, we can expect a variety of applications. For example, we here provide a stable tensor completion method, low-body tensor completion (LBTC). Traditional methods for tensor completion are based on the following iteration, called $em$-algorithm~\cite{WALCZAK200115}.

\begin{center} 
$e$-step: $\mathcal{P}_\Omega \leftarrow \mathcal{T}_{\Omega}$,
$m$-step : $\mathcal{P} \leftarrow$ \texttt{low-rank-approximation}$(\mathcal{P}), \quad $
\end{center} 

with initialized tensor $\mathcal{P}$ where $\Omega$ is observed indices of a given tensor $\mathcal{T}$ with missing values. 
From the information geometric view, $m$-step does $m$-projection onto the model manifold $\mathcal{B}$ consisting of low-rank tensors, and $e$-step does $e$-projection that finds the point on the data manifold $\mathcal{D}\equiv\set{\mathcal{P} \mid \mathcal{P}_{\Omega} = \mathcal{T}_{\Omega} }$ that minimizes the inverse KL divergence from a point on $\mathcal{B}$. The iteration of $e$- and $m$-step finds the closest point of $\mathcal{B}$ and $\mathcal{D}$. However, since low-rank subspace is not $e$-flat, that $m$-projection is not unique. %cannot find the global optimal solution. %As a result, the $em$-algorithms depends on initial positions. %Alternatively, recently, some methods have been developed to solve tensor completion with convex optimization by approximating ranks by trace norm~\cite{6138863}. However, these methods also require hyper-parameters that are time-consuming to tune.

LBTC conducts stable missing completion by replacing $m$-step with many-body approximation. The model manifold of many-body approximation is always $e$-flat and data manifold is $m$-flat. Since $em$-algorithm between $e$-flat and $m$-flat manifolds always converge~\citep[Chapter~1]{Amari16}, \emph{LBTC converges} as shown in Figure~\ref{fig:bands}(right). Instead of hyper-parameters that traditional tensor completion methods require, LBTC requires information about interactions to be used, but it can be intuitively tuned, as seen in Section~\ref{sec:demo}. 

==> tables/LBTC_scores.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\caption{Recovery fit score for tensor completion.}
      \label{tab:LBTC}
      \begin{tabular}{lccc}
        \toprule % <-- Toprule here
        \textbf{} & \textbf{Sce.~1 } & \textbf{Sce.~2} & \textbf{Sce.~3}\\
        %Missing ratio & 0.09 & 0.27 & 0.34 \\
        \midrule % <-- Midrule here
        LBTC & \textbf{0.948} & \textbf{0.917} & \textbf{0.873} \\
        HaLRTC          & 0.864 & 0.842 & 0.825 \\
        SiLRTC          & 0.863 & 0.841 & 0.820 \\
        SiLRTCTT       & 0.948 & 0.915 & 0.868 \\
        PTRCRW          & 0.945 & 0.901 & 0.844 \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
\end{wraptable}
